Densely Connected Graph Convolutional Networks for Graph-to-Sequence Learning

We focus on graph-to-sequence learning, which can be framed as transducing graph structures to sequences for text generation. To capture structural information associated with graphs, we investigate the problem of encoding graphs using graph convolutional networks (GCNs). Unlike various existing approaches where shallow architectures were used for capturing local structural information only, we introduce a dense connection strategy, proposing a novel Densely Connected Graph Convolutional Networks (DCGCNs). Such a deep architecture is able to integrate both local and non-local features to learn a better structural representation of a graph. Our model outperforms the state-of-the-art neural models significantly on AMRto-text generation and syntax-based neural machine translation.

==> tables/table2params.tex <==
\begin{table}[!t]
\centering
\small
\setlength{\tabcolsep}{1pt}
\begin{tabular}{lccclccc} 
\hline
\textbf{Model} & \texttt{D} & \texttt{\#P} & \texttt{B} & \textbf{Model} & \texttt{D} & \texttt{\#P} & \texttt{B} \\\hline
GCN(5) & 336 & 11.8M & 20.9 & GCN(4) & 372 & 11.8M & 18.3 \\
GCN(3) & 426 & 11.8M & 18.3 & GCN(2) & 486 & 11.7M & 18.2 \\
%\hline
DCGCN1 & 360 & 11.8M & \textbf{22.9} & & & & \\
\hline
GCN(10) & 336 & 14.0M & 21.3 & GCN(8) & 372 & 14.0M & 21.2 \\
GCN(6) & 426 & 14.0M & 21.5 & GCN(4) & 512 & 14.0M & 20.2\\
%\hline
DCGCN2 & 360 & 14.0M & \textbf{24.2} & & & & \\
\hline
GCN(15) & 336 & 16.3M & 19.9 & GCN(12) & 372 & 16.2M & 21.6 \\
GCN(9) & 426 & 16.2M & 22.1 & GCN(6) & 512 & 16.1M & 21.3 \\
%\hline
DCGCN3 & 360 & 16.2M & \textbf{24.8} & & & & \\
\hline
GCN(20) & 336 & 18.5M & 19.9 & GCN(16) & 372 & 18.4M & 20.6 \\
GCN(12) & 426 & 18.4M & 22.1 & GCN(8) & 512 & 18.2M & 21.8 \\
%\hline
DCGCN4 & 360 & 18.4M & \textbf{25.5} & & & & \\
\hline
\end{tabular}
\vspace{-1mm}
\caption{Comparisons with baselines. \text{DCGCN}$i$ represents our model with $i$ blocks. \text{GCN}($i$) represents GCNs with $i$ layers. All GCNs with both residual connections and layer aggregations. \texttt{D}: hidden dimension of the model. \texttt{\#P}: number of parameters. \texttt{B}: BLEU. }
\vspace{-3mm}
\label{tab:params}
\end{table}

==> tables/table7andfigure6.tex <==
\begin{figure}
\begin{floatrow}
\ffigbox{%
  \rule{3cm}{3cm}%
}{%
  \caption{A figure}%
}
\capbtabbox{%
  \begin{tabular}{cc} \hline
  Author & Title \\ \hline
  Knuth & The \TeX book \\
  Lamport & \LaTeX \\ \hline
  \end{tabular}
}{%
  \caption{A table}%
}
\end{floatrow}
\end{figure}
